Learning Robot Swarm Tactics over Complex Adversarial Environments

To accomplish complex swarm robotic missions in the real world, one needs to plan and execute a combination of single robot behaviors, group primitives such as task allocation, path planning, and formation control, and mission-specific objectives such as target search and group coverage. Most such missions are designed manually by teams of robotics experts. Recent work in automated approaches to learning swarm behavior has been limited to individual primitives with sparse work on learning complete missions. This paper presents a systematic approach to learn tactical mission-specific policies that compose primitives in a swarm to accomplish the mission efficiently using neural networks with special input and output encoding. To learn swarm tactics in an adversarial environment, we employ a combination of 1) map-to-graph abstraction, 2) input/output encoding via Pareto filtering of points of interest and clustering of robots, and 3) learning via neuroevolution and policy gradient approaches. We illustrate this combination as critical to providing tractable learning, especially given the computational cost of simulating swarm missions of this scale and complexity. Successful mission completion outcomes are demonstrated with up to 60 robots. In addition, a close match in the performance statistics in training and testing scenarios shows the potential generalizability of the proposed framework.

==> Fig/intro-kar.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sc:Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Swarm robotic systems promise new operational capabilities in uncertain, and often adversarial environments such as disaster response~\cite{matsuno2004rescue,ghassemi2019decmrta}, surveillance, and tactical assistance on battlefields. %In these contexts, swarm robots can offer task parallelism, efficiency, and fault-tolerance. 
Swarm systems require basic capabilities such as dynamically partitioning the swarm into groups, and commanding the groups to carry out different tasks that collectively ensure success of the mission. Adversarial environments present additional challenges to regular swarm applications because the swarms have to make tactical decisions such as opting for suboptimal choices to ensure safety and sacrificing part of the swarm for the success of the mission. 
%End-to-end operation of swarm systems in such applications require partitioning of the swarm into groups that are allocated different tasks, and executing diverse swarm primitives for collective motion and task execution. These requirements call for tactical planning capabilities to answer: i) when and how to sub-group, and ii) what task and associated primitive to be allocated to each sub-group. This paper develops a new learning-driven approach to perform real-time tactical planning for a heterogeneous swarm of autonomous unmanned ground and aerial vehicles which are conducting search missions in uncertain adversarial urban environments. We demonstrate that appropriate state abstraction and input/output encoding is key to learning robust, generalizable swarm tactics in realistic scenarios. 
Existing approaches for guiding swarm-level decision-making in complex environment can be broadly divided into handcrafted and automated approaches. Handcrafted approaches are algorithms for swarm deployment put together by an expert, and will require the expert for every new deployment/scenario. These have been shown to not be able to address several complexities and scale poorly wrt size of the swarm as well as application complexity and provide sub-optimal performance in real life \cite{AndrewIlachinski2017,brambilla2013swarm}. Automated approaches, such as the use of reinforcement learning and/or evolutionary computing to design swarm behavior, have mostly been limited to the design of individual swarm primitives such as formation control~\cite{huttenrauch2019deep}, coverage~\cite{jiang2020multi} and target tracking\cite{baldazo2019decentralized}.  These automated approaches have been restricted to small, homogenous teams of robots and relatively simple environments\cite{tan2013research, kim2016design,fan2017evolving,gajurel2018neuroevolution} as it is challenging to scale them up directly. 

%Handcrafted approaches, while good at creating new tactics, are unable to address multiple complexities, scale poorly with swarm size, and provide sub-optimal performance \cite{AndrewIlachinski2017,brambilla2013swarm}. Automated techniques, which are mostly based on reinforcement learning (RL) and evolutionary computing have been traditionally employed to optimize swarm behavior at the level of individual primitives such as formation flight, coverage, and target search~\cite{huttenrauch2019deep,jiang2020multi,baldazo2019decentralized}. Further, most reported demonstrations apply either to very small teams of robots or homogeneous swarms operating in relatively simple environments \cite{tan2013research, kim2016design,fan2017evolving,gajurel2018neuroevolution} and are challenging to scale up in either dimension.

%There is a growing body of work on tactical-level decision-making in the broader area of multi-agent systems and autonomous vehicles \cite{stodola2016tactical,mukadam2017tactical,hoel2020tactical,kokkinogenis2019tactical}, which use methods such as auction mechanisms and deep reinforcement learning. 
%Majority of these methods assume full observability across the swarm or multi-vehicle system, and do not provide any mechanism to consider adversarial units and their impact.   %In the current paper, we relaxed this assumption and considered a more uncertain environment. In addition to lack of observation, we assume adversarial units (both static and dynamic) against our heterogeneous team of robots. 
%
%This tactical decision-making should be applicable for a heterogeneous swarm that is operating in an uncertain and adversarial environment. One way of obtaining tactical policy is to apply optimization-based approaches. However, the tasks should be well modeled and adhere to strict, uncertain assumptions. 
%

Recently, deep RL has been applied to swarm systems \cite{huttenrauch2019deep} and related multi-vehicle problems \cite{stodola2016tactical,mukadam2017tactical,hoel2020tactical,kokkinogenis2019tactical}. Nonetheless, it remains challenging to tackle the large state spaces presented by large-scale swarms operating in complex environments involving obstacles and uncertain adversarial factors. Large input/output spaces, which demand large neural networks based policy models, are known to cause problems for RL approaches in general \cite{hinton2006reducing, lillicrap2015continuous,gueant2019deep}.
% \remove{Recent AI trends have seen modern methods from machine learning to various applications} \cite{kober2013reinforcement, jordan2015machine}. \remove{Attempting to learn swarm behavior comes with its own set of challenges.} 
%Given that each robot has several states (pose, sensors) that define the input to a learning system, a swarm's input space would be gigantic. The same problem exists for the actions of swarm members. This makes the problem extremely difficult for learning approaches, which have limitations to work with colossal input/output problem\cite{hinton2006reducing, lillicrap2015continuous,gueant2019deep}.
%
% Therefore, many approaches have been used to address this, such as hand-crafted methods \cite{liemhetcharat2015continuous,schwarzrock2018solving, and obute2019simple akrour2011preference, trianni2005emergent}.
% These methods generally use hand-coded algorithms and mechanisms with specific parameters and then tune these parameters through learning to obtain more efficient solutions. These parameters can be tuned using various optimization methods, depending on the application's nature and the hand-crafted algorithm. Some of these hand-coded algorithms are inspired by nature, using insect hive-mind behavior in ant or bee colonies. The different components that define the swarm's behavior can be tuned to allocate tasks in an efficient manner \cite{dantu2011programming,dantu2012comparison,fortino2014decentralized,khaluf2019local,arvin2014colias,alshawi2017minimal,zheng2010multi,halasz2007dynamic}. 
% These methods have more generalizability than non-nature-inspired methods due to their ability to change their behavior depending upon the environment. However, these methods are still limited to a set of rules defined by the algorithm. In contrast, machine learning can change the behavior and alter these rules entirely, resulting in potentially more adaptive and efficient solutions.
%

In this work, we demonstrate the use of artificial neural networks to design complex swarm operations at scale. We accomplish this through several innovations: \\
%\begin{itemize}
\underline{\it Group Abstraction}: A major challenge in observing the state of the swarm for control is an explosion of the state space. Motivated by grouping explosion strategy~\cite{zheng2013group}, we design our learning system to command groups instead of individual robots and thereby reduce the input complexity. \\
\underline{\it Toplogical Graph}: Similarly, continuous output spaces~\cite{smart2000practical} in swarm operations result in misleading, sparse or delayed reward functions~\cite{singh2009rewards} and costs that limit the number of learning samples~\cite{dulac2019challenges}. We address this problem by providing a topological graph abstraction, a much simpler representation of space that reduces the dimension of outputs.  \\
% command outputs.  \\
\underline{\it Pareto Optimality}: Further, we use Pareto optimality to creatively identify a smaller subset (of critical points of interest) in the action space for improved mission outcomes.\\
% \kar{someone say more?}\\
\underline{\it End-end Mission Rewards}: Given the uncertainty of each deployment as well as presence of adversaries, it is challenging to design consistent intermediate rewards during the mission. Therefore, we formulate end-of-mission rewards that closely align with mission objectives. \\
\underline{\it Neuroevolutionary Learning}: To make it all work, we leverage our prior work in neuroevolution~\cite{behjat2019adaptive} for improved performance in such uncertain scenarios.\\
% \kar{sentence or two on why AGENT is most suited for this learning}. \\
\underline{\it Novel Simulation Environment}: Given the end-of-mission nature of rewards, we needed a fast simulation environment for learning. We custom-built an environment that uses PyBullet for realistic physics and incorporates several open-source as well as custom implementations of swarm primitives (path planning, formation control, adversary avoidance) for group control. We provide an easy way to create and import topological maps for the output space abstraction in this simulator. Most importantly, our simulator runs much faster than real-time for quick learning, even at the scale of tens of robots and an area of hundreds of square meters.  
%\end{itemize}

%Our first approach to tackling the massive input-space problem is state-adaptive division of the swarm into groups (motivated by the grouping explosion strategy \cite{zheng2013group}). This provision to command groups instead of individual robots reduces the input/output dimensions of the learning problem. 

%Further challenges to learning tactics are presented by the need to handle continuous output spaces \cite{smart2000practical}, misleading, sparse or delayed reward functions \cite{singh2009rewards}, and simulation costs that limit the number of learning samples \cite{dulac2019challenges}. The last item is attributed to the significant expense of simulating (with acceptable realism) large swarms operating in complex environments. To tackle the problem of continuous outputs w.r.t. locations to visit within the urban environment, we define a topological graph that converts the continuous urban map into a small set of discrete choices that are applicable as actions to groups of robots. %This discretization is found to be more useful than space grid approaches, since the latter are difficult to adapt to complex urban environments. 
%While topological graph discretization decreases the action space, the number of nodes in the topological map \cite{kuipers1978modeling} might still be huge for larger urban environments, again putting significant burden on the learning process. 
%Subsequently, we use the concept of Pareto optimality to creatively skim out a smaller set of graph nodes that can be assigned as actions. Note that by discretizing and reducing the input/output spaces, we also reduce the size of the policy neural network model that needs to be trained, thereby alleviating the number of training episodes to be simulated. 

%Given the presence of uncertainties and adversities, it is challenging to assign intermediate rewards during the swarm mission. Instead, we formulate end-of-mission reward functions that closely align with the mission level objectives. Notably our preliminary experiments showed that such reward functions lead to gradient computations that might limit the performance of vanilla policy gradient implementations. Hence, we have employed a neuroevolution method that is less affected by the nature of the reward function, and provides other benefits such as ready parallelization, and the ability to evolve minimalist neural network topologies (as opposed to overtly large prescribed networks) that can yield generalizable performance over unseen scenarios.  %However, they are also more computationally expensive to assess \cite{o2016combining,gu2017deep}. To solve the computational expense issue, we use neuroevolution.% method - a particular variation called AGENT \cite{behjat2019adaptive}. 

%Evolutionary methods are less likely to remain trapped in local minima \cite{salimans2017evolution}. They can also be parallelized easily, which helps us achieve convergence sooner. Finally, to further help accelerate the function evaluation time, we develop a new multi fidelity swarm environment with full control of the simulation.

%The contributions of our work on learning-based swarm tactics generation can thus be summarized as follows: 
%\begin{itemize}
%    \item State abstraction of complex urban environments via graph encoding and clustering to dynamically group robots and embed state information over the graph, leading to a reduced I/O space for the tactics model.
%    \item Mission-adaptive Pareto encoding of outputs, leading to reduced set of tasks that can be allocated to individual groups or squads of robots.
%    \item Interfacing with the new I/O encoding methods, and exploring the effectiveness of, a recently developed neuroevolution algorithm for learning the tactics model.
%    \item A new Pybullet environment for simulating the swarm operations and demonstrating tactics; this simulation deploys both state-of-the-art and new primitives (e.g., path planning, formation control and adversary avoidance).
    %
    % \item We propose a novel architecture to learn swarm behavior using neuroevolution.
    % \item To reduce the learning problem's dimensionality, we perform learning on groups of robots and allow for dynamic regrouping.
    % \item We use a Pareto filter to decrease the resultant state-space to make the learning problem tractable.
    % \item We provide a framework applicable for many problems with heterogeneity, partial observation, and adversarial units.
    % \item We demonstrate our learned behavior in a relatively high fidelity environment with {up to 180} robots.
%\end{itemize} 
%
To demonstrate these contributions, we use the following prototypical swarm mission: deploy a swarm of $6-60$ UGVs and $12-120$ UAVs that search a realistic urban area spanning multiple blocks, to find the building (among multiple potential candidates) that contains a target, while tackling multiple squads of adversarial units that have the ability to engage and disable parts of the swarm. 

% {The proposed model can be useful in different applications beyond the application discussed here. For instance }

For the rest of the paper, we distinguish between {\it primitives} and {\it tactics} in swarm behavior design. We refer to single behaviors of a group as a primitive. Examples could be formation control, distributed mapping, group coverage and others. Tactics are ensembles of primitives commanded on multiple groups for swarm behavior. In this work, we assume that group primitives have been previously implemented and available for use. The objective of this work is thus to learn swarm tactics given the primitives for efficient swarm operation in presence of uncertainty and adversaries. 


% {\color{red} Rewrite the last two contributions to be more specific}
%The rest of this paper is outlined as follows: In section \ref{sec:Framework}, we introduce the overall framework and the learning method. In Section \ref{sec:Encoding}, we explain our state abstraction and input/output encoding. In Section \ref{sec:pybullet}, we describe the simulation environment. In Section \ref{sec:Problem_df}, we describe the swarm missions, and formulate the reward functions. In Section \ref{sec:results}, we present the results of our work, and concluding remarks are given in Section~\ref{sec:Conclusion}.



==> old/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
% \label{sc:Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\textcolor{mygreen}{Introduction structure -- swarm operation in complex uncertain (often adversarial) environment (for combat, disaster response, long-term extra-terrestrial exploration, etc.) requires a combination of multiple swarm algorithms or primitives, and sub-grouping of the swarm --> this calls for tactical decision-making to guide what primitive and associated task to allocate to sub-groups, how to sub-group, and when. ---> AI or ML is the way to go for tactical decision-making (which is mostly done by humans today, unless there are few papers on AI or some computation based tactical decision-making(then refer to that)). ---> to make learning, aka AI, tractable, we need encoding of state/action spaces (there is a lot of justification for this from the broader domain of AI applications in autonomous systems, robotics, bio-medicine, etc.) --> this brings us to the objectives or contributions of this paper.}
\end{comment}


Swarm robotic systems promise new operational capabilities in uncertain, and often adversarial environments such as disaster response~\cite{matsuno2004rescue,ghassemi2019decmrta}, peacekeeping, and extra-terrestrial exploration. %In these contexts, swarm robots can offer task parallelism, efficiency, and fault-tolerance. 
End-to-end operation of swarm systems in such applications require partitioning of the swarm into groups that are allocated different tasks, and executing diverse swarm primitives for collective motion and task execution. These requirements call for tactical planning capabilities to answer: i) when and how to sub-group, and ii) what task and associated primitive to be allocated to each sub-group. This paper develops a new learning-driven approach to perform real-time tactical planning for a heterogeneous swarm of autonomous unmanned ground and aerial vehicles which are conducting search missions in uncertain adversarial urban environments. We demonstrate that appropriate state abstraction and input/output encoding is key to learning robust, generalizable swarm tactics in realistic scenarios. 

Existing approaches for guiding swarm-level decision-making in complex environment can be broadly divided into handcrafted and automated approaches. Handcrafted approaches, while good at creating new tactics, are unable to address multiple complexities, scale poorly with swarm size, and provide sub-optimal performance \cite{AndrewIlachinski2017,brambilla2013swarm}. Automated techniques, which are mostly based on reinforcement learning (RL) and evolutionary computing have been traditionally employed to optimize swarm behavior at the level of individual primitives such as formation flight, coverage, and target search~\cite{huttenrauch2019deep,jiang2020multi,baldazo2019decentralized}. Further, most reported demonstrations apply either to very small teams of robots or homogeneous swarms operating in relatively simple environments \cite{tan2013research, kim2016design,fan2017evolving,gajurel2018neuroevolution} and are challenging to scale up in either dimension.

%There is a growing body of work on tactical-level decision-making in the broader area of multi-agent systems and autonomous vehicles \cite{stodola2016tactical,mukadam2017tactical,hoel2020tactical,kokkinogenis2019tactical}, which use methods such as auction mechanisms and deep reinforcement learning. 
%Majority of these methods assume full observability across the swarm or multi-vehicle system, and do not provide any mechanism to consider adversarial units and their impact.   %In the current paper, we relaxed this assumption and considered a more uncertain environment. In addition to lack of observation, we assume adversarial units (both static and dynamic) against our heterogeneous team of robots. 
%
%This tactical decision-making should be applicable for a heterogeneous swarm that is operating in an uncertain and adversarial environment. One way of obtaining tactical policy is to apply optimization-based approaches. However, the tasks should be well modeled and adhere to strict, uncertain assumptions. 
%
Recently, deep RL has been applied to swarm systems \cite{huttenrauch2019deep} and related multi-vehicle problems \cite{stodola2016tactical,mukadam2017tactical,hoel2020tactical,kokkinogenis2019tactical}. Nonetheless, it remains challenging to tackle the large state spaces presented by large-scale swarms operating in complex environments involving obstacles and uncertain adversarial factors. Large input/output spaces, which demand large neural networks based policy models, are known to cause problems for RL approaches in general \cite{hinton2006reducing, lillicrap2015continuous,gueant2019deep}.
% \remove{Recent AI trends have seen modern methods from machine learning to various applications} \cite{kober2013reinforcement, jordan2015machine}. \remove{Attempting to learn swarm behavior comes with its own set of challenges.} 
%Given that each robot has several states (pose, sensors) that define the input to a learning system, a swarm's input space would be gigantic. The same problem exists for the actions of swarm members. This makes the problem extremely difficult for learning approaches, which have limitations to work with colossal input/output problem\cite{hinton2006reducing, lillicrap2015continuous,gueant2019deep}.
%
% Therefore, many approaches have been used to address this, such as hand-crafted methods \cite{liemhetcharat2015continuous,schwarzrock2018solving, and obute2019simple akrour2011preference, trianni2005emergent}.
% These methods generally use hand-coded algorithms and mechanisms with specific parameters and then tune these parameters through learning to obtain more efficient solutions. These parameters can be tuned using various optimization methods, depending on the application's nature and the hand-crafted algorithm. Some of these hand-coded algorithms are inspired by nature, using insect hive-mind behavior in ant or bee colonies. The different components that define the swarm's behavior can be tuned to allocate tasks in an efficient manner \cite{dantu2011programming,dantu2012comparison,fortino2014decentralized,khaluf2019local,arvin2014colias,alshawi2017minimal,zheng2010multi,halasz2007dynamic}. 
% These methods have more generalizability than non-nature-inspired methods due to their ability to change their behavior depending upon the environment. However, these methods are still limited to a set of rules defined by the algorithm. In contrast, machine learning can change the behavior and alter these rules entirely, resulting in potentially more adaptive and efficient solutions.
%
Our first approach to tackling the massive input-space problem is state-adaptive division of the swarm into groups (motivated by the grouping explosion strategy \cite{zheng2013group}). This provision to command groups instead of individual robots reduces the input/output dimensions of the learning problem. 

Further challenges to learning tactics are presented by the need to handle continuous output spaces \cite{smart2000practical}, misleading, sparse or delayed reward functions \cite{singh2009rewards}, and simulation costs that limit the number of learning samples \cite{dulac2019challenges}. The last item is attributed to the significant expense of simulating (with acceptable realism) large swarms operating in complex environments. To tackle the problem of continuous outputs w.r.t. locations to visit within the urban environment, we define a topological graph that converts the continuous urban map into a small set of discrete choices that are applicable as actions to groups of robots. %This discretization is found to be more useful than space grid approaches, since the latter are difficult to adapt to complex urban environments. 
%While topological graph discretization decreases the action space, the number of nodes in the topological map \cite{kuipers1978modeling} might still be huge for larger urban environments, again putting significant burden on the learning process. 
Subsequently, we use the concept of Pareto optimality to creatively skim out a smaller set of graph nodes that can be assigned as actions. Note that by discretizing and reducing the input/output spaces, we also reduce the size of the policy neural network model that needs to be trained, thereby alleviating the number of training episodes to be simulated. 

Given the presence of uncertainties and adversities, it is challenging to assign intermediate rewards during the swarm mission. Instead, we formulate end-of-mission reward functions that closely align with the mission level objectives. Notably our preliminary experiments showed that such reward functions lead to gradient computations that might limit the performance of vanilla policy gradient implementations. Hence, we have employed a neuroevolution method that is less affected by the nature of the reward function, and provides other benefits such as ready parallelization, and the ability to evolve minimalist neural network topologies (as opposed to overtly large prescribed networks) that can yield generalizable performance over unseen scenarios.  %However, they are also more computationally expensive to assess \cite{o2016combining,gu2017deep}. To solve the computational expense issue, we use neuroevolution.% method - a particular variation called AGENT \cite{behjat2019adaptive}. 

%Evolutionary methods are less likely to remain trapped in local minima \cite{salimans2017evolution}. They can also be parallelized easily, which helps us achieve convergence sooner. Finally, to further help accelerate the function evaluation time, we develop a new multi fidelity swarm environment with full control of the simulation.

The contributions of our work on learning-based swarm tactics generation can thus be summarized as follows: 
\begin{itemize}
    \item State abstraction of complex urban environments via graph encoding and clustering to dynamically group robots and embed state information over the graph, leading to a reduced I/O space for the tactics model.
    \item Mission-adaptive Pareto encoding of outputs, leading to reduced set of tasks that can be allocated to individual groups or squads of robots.
    \item Interfacing with the new I/O encoding methods, and exploring the effectiveness of, a recently developed neuroevolution algorithm for learning the tactics model.
    \item A new Pybullet environment for simulating the swarm operations and demonstrating tactics; this simulation deploys both state-of-the-art and new primitives (e.g., path planning, formation control and adversary avoidance).
    %
    % \item We propose a novel architecture to learn swarm behavior using neuroevolution.
    % \item To reduce the learning problem's dimensionality, we perform learning on groups of robots and allow for dynamic regrouping.
    % \item We use a Pareto filter to decrease the resultant state-space to make the learning problem tractable.
    % \item We provide a framework applicable for many problems with heterogeneity, partial observation, and adversarial units.
    % \item We demonstrate our learned behavior in a relatively high fidelity environment with {up to 180} robots.
\end{itemize} 
%
To demonstrate these contributions, we use the following prototypical swarm mission: deploy a swarm of $6-60$ UGVs and $12-120$ UAVs that search for the building (among multiple potential candidates) that contains a target objective, while tackling multiple squads of adversarial units, in a complex environment spanning multiple urban blocks. 

% {The proposed model can be useful in different applications beyond the application discussed here. For instance }


% {\color{red} Rewrite the last two contributions to be more specific}
The rest of this paper is outlined as follows: In section \ref{sec:Framework}, we introduce the overall framework and the learning method. In Section \ref{sec:Encoding}, we explain our state abstraction and input/output encoding. In Section \ref{sec:pybullet}, we describe the simulation environment. In Section \ref{sec:Problem_df}, we describe the swarm missions, and formulate the reward functions. In Section \ref{sec:results}, we present the results of our work, and concluding remarks are given in Section~\ref{sec:Conclusion}.


